Multilingual Test-Time Scaling via Initial Thought Transfer

Test-time scaling has emerged as a widely adopted inference-time strategy for boosting reasoning performance. However, its effectiveness has been studied almost exclusively in English, leaving its behavior in other languages largely unexplored. We present the first systematic study of test-time scaling in multilingual settings, evaluating DeepSeek-R1-Distill-LLama-8B and DeepSeek-R1-Distill-Qwen-7B across both high- and low-resource Latin-script languages. Our findings reveal that the relative gains from test-time scaling vary significantly across languages. Additionally, models frequently switch to English mid-reasoning, even when operating under strictly monolingual prompts. We further show that low-resource languages not only produce initial reasoning thoughts that differ significantly from English but also have lower internal consistency across generations in their early reasoning. Building on our findings, we introduce MITT (Multilingual Initial Thought Transfer), an unsupervised and lightweight reasoning prefix-tuning approach that transfers high-resource reasoning prefixes to enhance test-time scaling across all languages, addressing inconsistencies in multilingual reasoning performance. MITT significantly boosts DeepSeek-R1-Distill-Qwen-7B's reasoning performance, especially for underrepresented languages.

==> ft_resource_llama_e3.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{ft_resource_llama_e3_raw.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> lang_id_1.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{lang_id_1_raw.pdf}
    \caption{Figure illustrates the }
    \label{fig:enter-label}
\end{figure*}

==> lang_id_1_granular.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{lang_id_1_granular_raw.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}

==> overall.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{overall_raw.pdf}
    \caption{Figure illustrates test-time scaling trends for \texttt{DeepSeek-R1-Distill-LLama-8B} \textbf{(a)} and \texttt{DeepSeek-R1-Distill-Qwen-7B} \textbf{(b)} for \texttt{AIME-2025-Contest-I} \textbf{(I)} and \texttt{AIME-2025-Contest-II} \textbf{(II)}. The results illustrate that \texttt{DeepSeek-R1-Distill-LLama-8B} shows robust progressive gains per scaling test-time compute unlike \texttt{DeepSeek-R1-Distill-Qwen-7B}}
    \label{fig:overall}
\end{figure*}

==> resource.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{resource_raw.pdf}
    \caption{Figure illustrates how the extent of test-time scaling varies with the resource availability of the target language in monolingual setting.  Languages are grouped into high-resource and low-resource categories, with separate curves plotted for each model: \texttt{DeepSeek-R1-Distill-LLaMA-8B} \textbf{(a)} and \texttt{DeepSeek-R1-Distill-Qwen-7B} \textbf{(b)}. The results reveal a consistent pattern: both models demonstrate stronger test-time scaling in high-resource languages compared to low-resource ones.\texttt{DeepSeek-R1-Distill-Qwen-7B} shows insignificant test-time scaling for low-resource languages.}
    \label{fig:resource}
\end{figure*}

==> result_initial_thought_similarity.tex <==
\section{Initial Thought Similarity Across Languages}
To counter the inconsistent test-time scaling trends for low-resource languages, we conduct a series of exploratory experiments to quantify differences in the multilingual reasoning scenarios concerning extremely complicated problems. Figure \ref{fig:similarity_initial_reasoning} illustrates the similarity of the initial reasoning segments pertaining to different languages to that of English for \texttt{DeepSeek-R1-Distill-Llama-8B} on \texttt{AIME-Contest-2025-I}A. Figure \ref{fig:similarity_initial_reasoning}(a) shows results using the multilingual embedder \texttt{paraphrase-multilingual-mpnet-base-v2} while Figure\ref{fig:similarity_initial_reasoning}(b) shows results after translating all reasoning segments to English and using \texttt{all-mpnet-base-v2} to measure similarity. Low-resource languages have increasingly dissimilar initial thoughts compared to English and other high-resource languages. This suggests a structural divergence in early reasoning strategies depending on language resource availability. The two-pronged evaluation methodology validates that these differences are not artifacts of embedding space mismatch or translation quality, but instead reflect deeper representational misalignment in multilingual model reasoning behaviors.

==> result_intervention.tex <==
\section{Intervention via Unsupervised Prefix-Tuning}

Motivated by previous trends of prefix similarity between high-resource and low-resource languages, we test if unsupervised prefix fine-tuning on English translates to enhancement of test-time scaling for reasoning. Figure \ref{fig:resource_qwen_e3} shows the results after training on each of 100 english reasoning prefixes for each question for both datasets. Unlike the inconsistent or flat trends seen in the base \texttt{DeepSeek-R1-Distill-Qwen-7B}, the fine-tuned model exhibits a clear upward trajectory with reasoning length — a hallmark of effective test-time scaling. Notably, this improvement is seen across both high-resource and low-resource languages, suggesting that English prefix tuning provides broadly transferable inductive priors for reasoning across the multilingual spectrum.


==> result_intra_inter.tex <==
\section{Intra- and Inter-Language Reasoning Prefix Similarity}

To further understand how the base steps of creating a reasoning solution differ for different languages, we sample 100 initial reasoning response prefixes (first 32 tokens) for each language and question pair. We measure the similarity of these reasoning solution prefixes by translating non-English prefixes to English and then utilizing \texttt{all-mpnet-base-v2}. The results in Figure \ref{fig:intra_prefix_similarity} reveal that low-resource languages tend to have lower intra-language similarity, indicating more variable early reasoning patterns, especially in \texttt{DeepSeek-R1-Distill-Qwen-7B}. In contrast, high-resource languages exhibit tighter and more consistent initial reasoning behaviors. These findings suggest that models demonstrate more stable inductive priors for high-resource languages.\par
For any two language pairs, we also measure the similarity between these reasoning prefixes and showcase the result averaged across all questions in Figure \ref{fig:inter_prefix_similarity}. The heatmaps reveal a clear pattern: high-resource languages exhibit stronger mutual similarity, indicating convergent early reasoning structures. In contrast, low-resource languages show weaker alignment, both with each other and with high-resource languages, especially in \texttt{DeepSeek-R1-Distill-Qwen-7B}.

==> result_language_mixing.tex <==
\section{Cross-lingual Leakage During Reasoning}
Deep diving into the quality of reasoning stream corresponding to each language, we test for any leakages into a foreign language. Figure \ref{fig:lang_id_2} shows the results for the two models under study. We observe that the 'thought-language' appears to change to `English' in different monolingual settings. This phenomenon is highly prevalent in \texttt{DeepSeek-R1-Distill-Llama-8B} as compared to \texttt{DeepSeek-R1-Distill-Qwen-7B}, which maintains the fidelity of the target language. Moreover, this phenomenon is seen to occur more in low-resource languages as compared to high-resource languages indicating the difficulty in maintaining long reasoning chains in a low-resource language.
